Uncertainty-Aware Candidate Generation for Entity Linking in Cyber Threat Intelligence

Entity Resolution (ER) pipelines often collapse ambiguity into early hard decisions: upstream Named Entity Recognition (NER) selects a single span and type, and downstream Entity Linking (EL) treats that choice as ground truth. This discards valuable information about the ambiguity of the underlying data (e.g., span boundary disagreement and type confusion), leading to brittle systems that fail unpredictably when faced with uncertainty in inputs. Therefore, this work presents a proof-of-concept for uncertainty-aware ER that treats uncertainty as native data that should be preserved and exploited throughout ER pipelines. We (i) capture uncertainty signals in the NER stage and (ii) leverage these signals into the EL stage to improve candidate retrieval under ambiguity. Using a BERT-based NER model augmented with two auxiliary span-boundary prediction heads, we apply Monte Carlo (MC) dropout at inference time to derive three mention-level proxy signals: the MC-averaged start-boundary probability, the MC-averaged end-boundary probability, and De Luca-Termini fuzzy entropy computed over the Begin-Inside-Outside (BIO) predictive distribution. These signals are used to adapt the fuzzy cutoff in candidate generation (CG) for EL. Because CG is treated as a blocking step, we evaluate retrieval recall. On the AnnoCTR dataset linked to the MITRE ATTCK knowledge base, the boundary-aware and dual-signal fuzzy linking approaches improve Recall@10 from 0.6186 to 0.7966. The contribution lies not in an end-to-end optimised ER pipeline but in establishing uncertainty preservation as a viable and beneficial component of ER pipelines, enabling downstream EL to make better-informed decisions under uncertainty.

==> Acknowledgements_CRediT.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{CRediT authorship contribution statement}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

